(Almost Full) EFX Exists for Four Agents (and Beyond)

The existence of EFX allocations is a major open problem in fair division, even for additive valuations. The current state of the art is that no setting where EFX allocations are impossible is known, and EFX is known to exist for ($i$) agents with identical valuations, ($ii$) 2 agents, ($iii$) 3 agents with additive valuations, ($iv$) agents with one of two additive valuations and ($v$) agents with two-valued instances. It is also known that EFX exists if one can leave $n-1$ items unallocated, where $n$ is the number of agents. We develop new techniques that allow us to push the boundaries of the enigmatic EFX problem beyond these known results, and, arguably, to simplify proofs of earlier results. Our main results are ($i$) every setting with 4 additive agents admits an EFX allocation that leaves at most a single item unallocated, ($ii$) every setting with $n$ additive valuations has an EFX allocation with at most $n-2$ unallocated items. Moreover, all of our results extend beyond additive valuations to all nice cancelable valuations (a new class, including additive, unit-demand, budget-additive and multiplicative valuations, among others). Furthermore, using our new techniques, we show that previous results for additive valuations extend to nice cancelable valuations.

==> Inputs/0.Tasks.tex <==

%%%%%%%%%% NOTES FOR INTERNAL USE %%%%%%%%%%%%%


\section{Section 0: to be removed.}
\subsection{Tasks}
\begin{itemize}
	\item Proofread all sections (especially 4 player 1 unalloc result): make sure everything is understandable.
	\item Proofread envy result.
	\item Take care of structure in all sections (put things into claims, lemmas)
	\item \sout{Rewrite n-2 section:  remove def of colorful cycle (this is a basic PI cycle now), change and shorten statements and proofs accordingly.  Graph theoretic lemma should focus on $M_\allocs$, etc.}
	\item \sout{Take care of agents not envying the charity, in all results.}
	\item Remove all \cancbty| + Observation \ref{obs:T_k<T_j} explanations?
	\item Abstract.
	\item Ben+Avi:  go over intro.
	\item \sout{Remove RC instances: switch with cancelable.}
	\item Take care of handwritten squares in envy section of 4 players result.
	\item Decide on cup vs. cupdot.  Low priority.  Uniformity not that important.
%	\item \sout{Transform every $i \champ[B_k \mid\circ] j$ to  vs. $i \champ[B_k \mid \circ] j$.}
	\item Make sure the citations in the intro are correct. I might have mixed up the two 2020 papers. (Michal)
	\item Add all missing references and citations to intro.
	\item \sout{Fix the proof of budget additive (make it more general).}
	\item Take care of figures:  %incorporate Karin's ppt.
		\begin{itemize}
			\item \sout{Remove $4\champ[\h]3$ edge in right figure in page 33 (Case \circled{II})}
			\item \sout{Remove Z self loop in Case \circled{II} in the envy section.}
			\item Change 2cm height to scaling in all figures.
		\end{itemize}
	
	\item Transfer to EC format.
	\item Think of ways to make everything more concise and clean.
	\item Think of what can be done to save space (remove wasteful definitions, bullets, etc.)
	\item \sout{Rewrite the proof for three players using updated setup.}
	\item Think of title.
	\item \sout{Acknowledge Karin, Chaudhury et al.} 
\end{itemize}


